Distance Estimation Between Unknown Matrices Using Sublinear Projections on Hamming Cube

Using geometric techniques like projection and dimensionality reduction, we show that there exists a randomized sub-linear time algorithm that can estimate the Hamming distance between two matrices. Consider two matrices ${\bf A}$ and ${\bf B}$ of size $n \times n$ whose dimensions are known to the algorithm but the entries are not. The entries of the matrix are real numbers. The access to any matrix is through an oracle that computes the projection of a row (or a column) of the matrix on a vector in $\{0,1\}^n$. We call this query oracle to be an {\sc Inner Product} oracle (shortened as {\sc IP}). We show that our algorithm returns a $(1\pm \epsilon)$ approximation to ${{\bf D}}_{\bf M} ({\bf A},{\bf B})$ with high probability by making ${\cal O}\left(\frac{n}{\sqrt{{{\bf D}}_{\bf M} ({\bf A},{\bf B})}}\mbox{poly}\left(\log n, \frac{1}{\epsilon}\right)\right)$ oracle queries, where ${{\bf D}}_{\bf M} ({\bf A},{\bf B})$ denotes the Hamming distance (the number of corresponding entries in which ${\bf A}$ and ${\bf B}$ differ) between two matrices ${\bf A}$ and ${\bf B}$ of size $n \times n$. We also show a matching lower bound on the number of such {\sc IP} queries needed. Though our main result is on estimating ${{\bf D}}_{\bf M} ({\bf A},{\bf B})$ using {\sc IP}, we also compare our results with other query models.

==> appln.tex <==
\section{Applications}\label{sec:appln}

==> back.tex <==
section{Proof of Lemma~\ref{lem:distrows} and Lemma~\ref{lem:almost}}
\label{sec:append-est-dist}
\noindent
%%%%%%%%%%%%%%%%%%%%%Start of proof of Lemma %%%%%%%%%%%%%
 \begin{lem}[Lemma~\ref{lem:distrows} restated]
 Consider \iporacle access to two  $n\times n$ (unknown) matrices $\mtx{A}$ and $
 \mtx{B}$. There is an algorithm $\distrows (i,\alpha,\delta)$ that takes $i\in [n]
 $ and $\alpha ,\delta\in (0,1)$ as inputs, reports a $(1\pm \alpha)$-approximation 
 to $\ham\left(\mtx{A}({i,*}),\mtx{B}({i,*})\right)$  with 
 probability at least $1-\delta$, and makes $\Oh\left(\frac{1}{\alpha^2} \log ^4 n \log 
 \frac{1}{\delta}\right)$ \iporacle queries to both $\mtx{A}$ and $\mtx{B}$.
 \end{lem}

 As noted in Section~\ref{sec:prelim}, $\distrows (i,\alpha,\delta)$ makes repeated calls to $\ident \left(S,i,\kappa\right)$ (the algorithm corresponding to Observation~\ref{obs:algo-zero}). We prove an intermediate result, that will be needed in our algorithm $\distrows (i,\alpha,\delta)$, stated as follows.
 
 \begin{lem}\label{lem:exact}
 Consider \iporacle access to two  $n\times n$ (unknown) matrices $\mtx{A}$ and $
 \mtx{B}$. There is an algorithm $\exact (S,i,\delta)$ that takes $S \subseteq [n]$, $i\in [n]
 $ and $\delta\in (0,1)$ as inputs, finds the exact value of $\ham\left(\mtx{A}({i,*})~\vert_S,\mtx{B}({i,*})~\vert_S\right)$, and makes $\Oh\left(\ham\left(\mtx{A}({i,*})~\vert_S,\mtx{B}({i,*})~\vert_S\right)\cdot \log n \cdot \log \frac{1}{\delta}\right)$. \iporacle queries to both $\mtx{A}$ and $\mtx{B}$. %Moreover, in case $\ham\left(\mtx{A}({i,*}),\mtx{B}({i,*})\right) \leq \tau$, the algorithm reports the exact value of $\ham\left(\mtx{A}({i,*})~\vert_S,\mtx{B}({i,*})~\vert_S\right) \leq \tau$.
 \end{lem} 
 \begin{proof}
For simplicity of presentation, we prove for the spacial case $S=[n]$. However. the proof for general $S$ is similar. 

We initialize a tree ${\cal T}$ with $[n]$ as the root. We build the tree such that each node is labeled with either $0$ or $1$. First we check if $\ham\left(\mtx{A}({i,*})~\vert_S,\mtx{B}({i,*})~\vert_S\right)=0$ by calling $\ident ([n],i, \frac{\delta}{n})$. If $\ham\left(\mtx{A}({i,*})~\vert_S,\mtx{B}({i,*})~\vert_S\right)=0$, we label the root with $0$ and terminate. Otherwise, we label the root with $1$ and do the following as long as there is a leaf node $X \subseteq [n]$ labeled with $1$.
\begin{itemize}
\item[(i)] We check if $\ham\left(\mtx{A}({i,*})~\vert_X,\mtx{B}({i,*})~\vert_X\right)=0$ by calling $\ident ([n],i, \frac{\delta}{n})$. If $\ham\left(\mtx{A}({i,*})~\vert_X,\mtx{B}({i,*})~\vert_X\right)=0$, then we label $X$ with $0$ and go to other leaf node labeled as $1$ if any. Otherwise, we label $X$ as $1$ and do the following.
\item[(ii)] If $\size{X}=1$, then we add one node as a child of $X$ and label the new node as $0$. Then we go to other leaf node labeled as $1$ if any.
\item[(iii)]  If $\size{X}\geq 2$, then we partition the set $X$ into $X_1$ and $X_2$; respectively, such that
   $\size{X_1}=\lceil \frac{\size{X}}{2} \rceil$ and $\size{X_2}=\lfloor \frac{\size{X}}{2} \rfloor$. We add $X_1$ and $X_2$ as two children of $X$.

\end{itemize}
Let $\cT'$ be the tree after deleting all the leaf nodes in $\cT$. Observe that $\ham\left(\mtx{A}({i,*})~\vert_S,\mtx{B}({i,*})~\vert_S\right)=0$ is the number of  leaf nodes in $\cT'$; and
\begin{itemize}
\item The height of ${\cal T}$ is bounded by $\log_2 \size{S}  \leq \log_2 n  $,
\item  The query complexity of the above procedure is bounded by the of nodes in ${\cal T}$ times $q$, where $q$ be the upper bound on number of \iporacle{} queries made by any call to $\ident ([n],i, \frac{\delta}{n})$. This is  as we make at most one query per node of $\cT$,
%\item $t(U,V,W)$ is bounded by the number of leaf nodes and the number of leaf nodes is bounded by $8 t(U,V,W)$.
\end{itemize}
%The number of nodes in $\cT'$, the number of internal nodes of $\cT$, is bounded by $2  \log n$. So,  the number of leaf nodes in $\cT$ is at most $16t(A,B,C) \log n$ and hence the total number of nodes in $\cT$ is at most $16t(U,V,W) \log n$. Putting everything together, the required query complexity is $\Oh(t(A,B,C)\log n)$. 
 \end{proof}
 
  \begin{lem}\label{lem:ths}
 Consider \iporacle access to two  $n\times n$ (unknown) matrices $\mtx{A}$ and $
 \mtx{B}$. There is an algorithm $\exact (S,i,\tau,\alpha,\delta)$ that takes $i\in [n]
 $, $\tau \in \N$, and $\alpha ,\delta\in (0,1)$ as inputs, decides whether  $\ham\left(\mtx{A}({i,*})~\vert_S,\mtx{B}({i,*})~\vert_S\right) \leq \tau$ or not  with 
 probability at least $1-\delta$, and makes $\Oh\left(\tau \log n \log \frac{1}{\delta}\right)$ \iporacle queries to both $\mtx{A}$ and $\mtx{B}$. Moreover, in case $\ham\left(\mtx{A}({i,*}),\mtx{B}({i,*})\right) \leq \tau$, the algorithm reports the exact value of $\ham\left(\mtx{A}({i,*})~\vert_S,\mtx{B}({i,*})~\vert_S\right) \leq \tau$.
 \end{lem}
 \begin{proof}
 
 \end{proof}
 
 
  Let us consider a random $R \subseteq [n]$ generated by including each $i \in [n]$ in $R$ with probability $\frac{1}{2^k}$. Note that $\E[\ham\left(\mtx{A}({i,*})~\vert_R,\mtx{B}({i,*})~\vert_R\right)]=\frac{\ham\left(\mtx{A}({i,*}),\mtx{B}({i,*})\right)}{2^k}$. Applying Chernoff bound (See Lemma~\ref{lem:chernoff}), for $\zeta \in (0,1)$ we get 
$2^k\ham\left(\mtx{A}({i,*})~\vert_R,\mtx{B}({i,*})~\vert_R\right)$ is an $(1 \pm 
\zeta)$-approximation to $\ham\left(\mtx{A}({i,*}),\mtx{B}({i,*}\right)$ with probability 
at least $1-\delta'$ 
%where $\delta' \leq\exp{\left(-\frac{\zeta^2}{3}\frac{\ham
%\left(\mtx{A}({i,*}),\mtx{B}(i,*)\right)}{2^k}}$.
\section{Proof of Lemma~\ref{lem:dist-res}}
\label{sec:append-sample-almost}
\noindent  
To prove Lemma~\ref{lem:almost}, we need notions of \emph{hierarchical subsets} of $[n]$  defined in Definition~\ref{defi:hset} and an observation (Observation~\ref{obs:hset}) about hierarchical subsets.

  \begin{lem}[Lemma~\ref{lem:almost} restated]
 Consider \iporacle{} access to two  $n\times n$ (unknown) matrices $\mtx{A}$ and $\mtx{B}$. \remove{Also, for $i\in [n]$, $\mbox{{\sc NEQ}}(\mtx{A},\mtx{B},i)$ denotes the set $\{j:\mtx{A}(i,j)\neq\mtx{B}(i,j)\}$.} There exists an algorithm $\randsamp(i,\alpha,\delta)$, described in Algorithm~\ref{algo:random-samp}, that takes $i \in [n]$ and $\alpha ,\delta\in (0,1)$ as input, reports a $(1\pm \alpha)$-uniform sample from the set $\mbox{{\sc NEQ}}(\mtx{A},\mtx{B},i)$ with probability at least $1-\delta$, and makes $\Oh\left(\frac{1}{\alpha^2} \log \frac{n}{\delta}\right)$ \iporacle queries to both $\mtx{A}$ and $\mtx{B}$.
 \end{lem}



\begin{defi}[{\bf Hierarchical subsets}]\label{defi:hset}
For $j\in [\log n]\cup \{0\}$, the $k$-th with $k\in \left[2^j\right]$ hierarchical subset of label $j$ is denoted and defined as $S_{j}^k=\{(k-1)\frac{n}{2^j}+1,\ldots,k\frac{n}{2^j}\}$. The set of \emph{hierarchical} subsets of $[n]$ with label $j$ is denoted and defined as $\cH_j=\{S_{j,k}:k\in \left[2^j\right]\}$. The set of hierarchical subsets of $[n]$ is denoted an defined as by $\cH= \bigcup\limits_{j=0}^{\log n}\cH_j=\{S_{j}^k:j\in [\log n]\cup \{0\}~\mbox{and}~k\in \left[2^j\right]\}$.  
 \end{defi}
 \begin{obs}\label{obs:hset}
Consider the set of hierarchical subsets $\cH$ of $[n]$ defined as above. Then
\begin{itemize}
\item[(i)] $\size{\cH}=2n-1$;
\item[(ii)] For any $j\in [\log n]\cup \{0\}$, the set of hierarchical subsets of label $j$ forms a partition of $[n]$;
\item[(iii)] For every $j \in [\log n-1]\cup \{0\}$ and $k \in [2^j]$, the $k$-th hierarchical subset in label $j$ is the disjoint union of two hierarchical subsets, that is, $(2k-1)$-th and $2k$-th hierarchical subset of label $j$. In other words,
$S_{j}^k=S_{j+1}^{2k-1} \sqcup S_{j+1}^{2k}$; 
\item[(iv)] For any $\ell \in [n]$ and for any $j\in [\log n]\cup \{0\}$, there is exactly one $k_j \in [2^j]$ such that $\ell$ is present in the $k_j$-th hierarchical subset of label $j$, that is, in $S_{j}^{k_j}$. Let $I(j,\ell)\in [2^j]$ be such that such that $I(j,\ell)$-th hierarchical subset of label $j$ has $\ell$ in it. 
\item[(v)] $I({\log n},\ell)=\ell$;
\item[(vi)]  For any $j\in [\log n-1]\cup \{0\}$, $I(j,\ell)=2I(j-1,\ell)-1$ or $I(j,\ell)=2I(j-1,\ell)$. That is, $I(j-1,\ell)=\lceil \frac{I(j,\ell)}{2} \rceil $.

%If $\ell$ in present in $k_j$-th and $k_{j+1}$-th subset of label $j$ and label $j+1$, respectively, then $k_{j+1}=2k_j$ or $k_{j+1}=2k_j-1$, that is, $k_j=\lceil \frac{k_{j+1}}{2}\rceil$.
\end{itemize}
 \end{obs}
 Apart from Definition~\ref{defi:hset} and Observation~\ref{obs:hset}, we also need the notion of \emph{projecting a vector in $\{-1,1\}^n$ into a set $S \subseteq [n]$} as defined in Definition~\ref{defi:hvec}.
 %below and an observation (Observation~\ref{obs:ip-eval}) about it. 
\remove{ \begin{defi}[{\bf Vector projeted into a set}]\label{defi:hvec}
 Let $\mtx{A}$ be a  $n\times n$ matrix and $i \in [n]$. For $S\subseteq [n], \mtx{A}(i,*)~\vert_S \in \{0,1\}^n$ is defined as the vector having $\ell$-th coordinate equals to $\mtx{A}(i,\ell)$ if $\ell \in S$, and $0$, otherwise.
Also consider ${\bf r}\in \{-1,1\}^n$ and a set $S\subseteq [n]$. Then the vector ${\bf r}$ projected into $S$ is denoted ${\bf r}\vert_S \in \{-1,0,1\}^n$ and defined as follows: For $\ell \in [n]$, the $\ell$-th coordinate of ${\bf r} \vert_S$ is same as that of ${\bf r}$ if $\ell \in S$, and $0$, otherwise.

 \end{defi}
%Note that $\size{\cH}=2n-1$ and $\size{\cV_{\cH}({\bf A},i)}=2n-1$. 
 \begin{obs}\label{obs:ip-eval}
Let $\mtx{A}$ be a  $n\times n$ matrix, $i \in [n]$, ${\bf r} \in \{-1,1\}^n$ and $S \subseteq [n]$. Then $\dpd{\mat{A}(i,*)\vert_S}{{\bf r}}=\dpd{\mat{A}(i,*)}{{\bf r}\vert_S}$. That is, $\dpd{\mat{A}(i,*)}{{\bf r}\vert_S}$ can be evaluated by using a \iporacle query $\dpd{\mat{A}(i,*)}{{\bf r}\vert_S}$ to matrix $\mat{A}$.
 \end{obs}}
 \comments{To prove Lemma~\ref{lem:almost}, we need the following intermediate lemma that says that the distance, between a row vector of $\mat{A}$ projected into a set $S \subseteq [n]$ with the corresponding row vector of $\mat{B}$ projected into $S$, can be approximated. The proof follows from Proposition~\ref{pre:JL} and Remark~\ref{rem:map}.}
 
 \begin{lem}[Lemma~\ref{lem:dist-res} restated]
 Consider \iporacle{} access to two  $n\times n$ (unknown) matrices $\mtx{A}$ and $\mtx{B}$. There exists an algorithm $\resdistrows (S,i,\alpha,\delta)$ that takes $S \subseteq [n]$, $i \in [n]$ and $\alpha ,\delta\in (0,1)$ as inputs, reports an $(1\pm \alpha)$-approximation to $\ham\left(\mtx{A}({i,*})~\vert_S,\mtx{B}({i,*})~\vert_S\right)$ with probability at least $1-\delta$, and makes $\Oh\left(\frac{1}{\alpha^2} \log^4 n \log \frac{1}{\delta}\right)$ many \iporacle queries to both $\mtx{A}$ and $\mtx{B}$. 
 \end{lem}
 \remove{
 \begin{lem}[{\bf Distance between hierarchical vectors}]\label{lem:dist-res}
 Consider \iporacle{} access to two  $n\times n$ (unknown) matrices $\mtx{A}$ and $\mtx{B}$. Also let $\cH$ denote hierarchical subset of $[n]$. There exists an algorithm $\resdistrows (S,i,\alpha,\delta)$ that takes $S \in \cH$, $i \in [n]$ and $\alpha ,\delta\in (0,1)$ as inputs, reports an $(1\pm \alpha)$-approximation to $\ham\left(\mtx{A}({i,*})~\vert_S,\mtx{B}({i,*})~\vert_S\right)$ with probability at least $1-\delta$, and makes $\Oh\left(\frac{1}{\alpha^2} \log \frac{1}{\delta}\right)$ many \iporacle queries to both $\mtx{A}$ and $\mtx{B}$.
 \end{lem}
 \begin{proof}
 The proof is similar to that of Lemma~\ref{lem:distrows}. Algorithm $\resdistrows (S,i,\alpha,\delta)$ finds ${\bf r_1},\ldots,{\bf r_d} \in \{-1,1\}^n$ such that each coordinate of every 
 ${\bf r_j}$ is taken from $\{-1,1\}$ uniformly at random where $d=\Theta\left(\frac{1}
 {\alpha^2}\log \frac{1}{\delta}\right)$. Then the algorithm finds $a_j=\dpd{\mat{A}(i,*)\vert_S}{{\bf r_j}}$ and  $b_j=\dpd{\mat{B}
 (i,*)\vert_S}{{\bf r_j}}$ by making one \iporacle query to each of $\mat{A}$ and $\mat{B}$. This is possible by Observation~\ref{obs:ip-eval}. Then the algorithm reports $||{\bf a}-{\bf b}||_2^2$ as an $\left(1 
 \pm \alpha \right)$-approximation to $\ham\left(\mtx{A}({i,*})\vert_S, \mtx{A}({i,*})\vert_S \right)$. 
 The query complexity of $\resdistrows (S,i,\alpha,\delta)$ is $2d=\Theta
 \left(\frac{1}{\alpha^2}\log \frac{1}{\delta}\right)$. The correctness of the 
 algorithm follows from Proposition~\ref{pre:JL} and Remark~\ref{rem:map}.
 
 %By Proposition~\ref{pre:JL} and Remark~\ref{rem:map}, $,\mtx{B}({i,*}\vert_S)\right)$ with probability at least $1-\delta$.  
 
 
 %We will be done with the proof by explaining how $\resdistrows (S,i,\alpha,\delta)$ finds $a_j$'s and $b_j$'s. ${\bf r_1}',\ldots,{\bf r_d}' \in \{-1,1\}^n$ such that ${\bf r_j}'={\bf r_j}$ if $j \in S$ and $0$, otherwise. Observe that, for each $j\in [d]$,  and $b_j=\dpd{\mat{B}(i,*)\vert_S}{{\bf r_j}}=\dpd{\mat{B}(i,*)}{{\bf r_j}'}$.
 
 
 \end{proof} }
 Now, we have all intermediate stuffs to show Lemma~\ref{lem:almost}. %For a set $S$ in the set $\cH$ of hierarchical subsets, let us define $\mbox{{\sc NEQ}}(\mat{A},\mat{B},S,i)=\mbox{{\sc NEQ}}(\mat{A},\mat{B},i)\cap S$
 \begin{algorithm}
\caption{$\randsamp \left(i,\alpha,\delta \right)$: Algorithm for sampling an $(1 \pm \alpha )$-approximation sample from $\mbox{{\sc NEQ}}(\mtx{A},\mtx{B},i)$.}
\label{algo:random-samp}
\KwIn{\iporacle access to unknown matrices $\mtx{A}$ and $\mtx{B}$, parameters $i\in [n]$ and $\alpha \in (0,1)$.}
\KwOut{An $(1 \pm \alpha)$-approximation sample from $\mbox{{\sc NEQ}}(\mtx{A},\mtx{B},i)$.}
Set $\alpha'=\frac{\alpha}{50 \log n}$ and $\delta'=\frac{\delta}{50 \log n}$.
%Call $\resdistrows \left(S_{0}^1,i,\alpha',\delta'\right)$ and let $d_0^1$ be the output.//$S_{0}^{1}=[n]$ is the first and only set having label $0$ in the set $\cH$ of hierarchical subsets of $[n]$.

Set $k_{0}=1$

\For{($j=1$ to $\log n$)}
{
Call $\resdistrows \left(S_{j}^{2k_{j-1}-1},i,\alpha',\delta'\right)$ and $\resdistrows \left(S_{j-1}^{2k_{j-1}},i,\alpha',\delta',\right)$. Let $d_1^j$ and $d_2^j$ be the respective outputs.
// $\resdistrows \left(S_{j}^{2k_{j-1}-1},i,\alpha',\delta'\right)$ is the algorithm as stated in Lemma~\ref{lem:dist-res}.

// Note that $S_{j}^{2k_{j-1}-1}$ and $S_{j}^{2k_{j-1}}$ are $(2k_{j-1}-1)$-th and $2k_j$-th hierarchical subsets of $[n]$ (See Definition~\ref{defi:hset}). 

%Let $d_{j-1}^{k_{j-1}}$ be the output of the call to $\resdistrows \left(S_{j-1}^{k_{j-1}},i,\alpha',\delta'\right)$ in the previous iteration.
 Set $k_j=2k_{j-1}-1$ with probability $\frac{d_1^j}{d_1^j+d_2^j}$ and $k_j$ with the remaining probability.
}
Report $k_{\log n}$ as the output.
\end{algorithm}
\begin{proof}[Proof of Lemma~\ref{lem:almost}]
Algorithm $\randsamp(i,\alpha,\delta)$  sets $\alpha'=\frac{\alpha}{10 \log n}$ and $\delta'=\frac{\delta}{50 \log n}$ and goes over $\log n$ many iterations. In the first iteration, it calls for $\resdistrows \left(S_{1}^{1},i,\alpha',\delta'\right)$ and $
\resdistrows \left(S_{1}^{2},\alpha',\delta',i\right)$. Let $d_{1}^{1}$ and $d_{1}
^{2}$ be the respective outputs. Then we select $S_1^1$ with probability $
\frac{d_1^1}{d_1^2+d_2^1}$ and on $S_1^2$ with the remaining probability. The algorithm sets $k_1=1$ or $2$ (as an indicator of which subset out of $S_1^1$ and $S_1^2$ is selected) depending on whether $S_1^1$ or $S_1^2$ is selected, and recurse on the selected subset in the second iteration. In the $j$-th iteration, note that, the algorithm calls $\resdistrows \left(S_{j}^{2k_{j-1}-1},i,\alpha',\delta'\right)$ and $\resdistrows \left(S_{j}^{2k_{j-1}},i,\alpha',\delta',\right)$. Let $d_1^j$ and $d_2^j$ be the respective outputs. Note that $S_{j}^{2k_{j-1}-1}$ and $S_{j}^{2k_{j-1}}$ are $(2k_{j-1}-1)$-th and $2k_j$-th hierarchical subsets of $[n]$ (See Definition~\ref{defi:hset}). The algorithm selects $S_j^{2k_{j-1}-1}$ with probability $\frac{d_1^j}{d_1^j+d_2^j}$ and $S_{j}^{2k_j}$ with the remaining probability. Then the algorithm sets $k_j=2k_{j-1}-1$ and $k_j=2k_{j-1}$ as an indicator of which set out of 
$S_{j}^{2k_j-1}$ and $S_j^{2k_j}$ is selected.
After executing all the $\log n$ iterations, $\randsamp \left(i,\alpha,\delta \right)$ reports $k_{\log n}$ as the output. A psedocode for $\randsamp(i,\alpha,\delta)$ is given in Algorithm~\ref{algo:random-samp}.



 $\randsamp(i,\alpha,\delta)$ calls for $\resdistrows(S,i,
\alpha',\delta')$ $2\log n-1$ times in total by taking different parameters in 
place of $S$. By Lemma~\ref{lem:dist-res}, we make $\Oh \left(\frac{1}{(\alpha')^2} \log \frac{1}\delta'\right)$ many \iporacle queries to matrices $\mat{A}$ and $\mat{B}$. So, the total number of \iporacle queries made by $\randsamp(i,\alpha,\delta)$ is $\Oh \left(\frac{\log ^3 n}{\alpha^2}\log \frac{n}{\delta}\right)$. Let $\cE$ be the event that all the calls to $\resdistrows$ gives 
desired output. Observe that $\Pr(\cE) \geq 1-\delta'(2\log n-1) \geq 1-\delta$. 
We show the correctness proof for $\randsamp(i,\alpha,\delta)$ on the conditional space that $\cE$ holds. Particularly, we will show that the algorithm returns an $(1 \pm \alpha)$-
approximate sample from set $\mbox{{\sc NEQ}}(\mat{A},\mat{B},i)$ when $\cE$ holds. From the description of Algorithm~\ref{algo:random-samp}, $k_{\log n}$ is the output which is a random variable. In what follows, we will show that $k_{\log n}$ is an $\left(1 \pm \alpha \right)$-approximate sample from $\mbox{{\sc NEQ}}(\mat{A},\mat{B},i)$, that is, for any $\ell \in \mbox{{\sc NEQ}(\mat{A},\mat{B})}$,

\begin{equation}
 (1-\alpha)\frac{1}{\size{\mbox{{\sc NEQ}(\mat{A},\mat{B},i)}}} \leq \pr(k_{\log n}=\ell) \leq (1+\alpha)\frac{1}{\size{\mbox{{\sc NEQ}(\mat{A},\mat{B},i)}}}.
 \end{equation}

 

From Observation~\ref{obs:hset} (iv), recall that $I(j,\ell)\in [2^j]$ be such that such that $I(j,\ell)$-th hierarchical subset of label $j$ has $\ell$ in it. Moreover, $I(\log n,\ell)=\ell$ by Observation~\ref{obs:hset} (v). So, we approximate the probability of the event $k_{\log n}=I(\log n,\ell)$ instead of $k_{\log n}=\ell$. Consider the following observation that follows from the description of our algorithm along with Observation~\ref{obs:hset}.

\begin{obs}\label{obs:sampled-all}
\begin{itemize}
\item[(i)] $k_{\log n}=\ell$ if and only if $k_{j}=I(j,\ell)~\forall ~j \in [\log n]\cup \{0\}$;
\item[(ii)] In general, for any $j\in [\log n]$, $k_{j}=I(j,\ell)$ if and only if $k_{j'}=I(j',\ell)~\forall ~j' \in [j]$.
\end{itemize}
\end{obs}
Note that our target is to approximate $\pr\left(k_{\log n}=I(\log n, \ell)=\ell 
\right)$. To do so, $\pr\left(k_{\log n}=\ell\right)$, consider $E_j$, where $j 
\in [\log n] \cup \{0\}$, that denotes the event that $k_j=I(j,\ell)$. 
By Observation~\ref{obs:sampled-all},
\begin{equation}\label{eqn:prob-cond}
 \pr \left( k_{\log n} = \ell \right) = \pr \left( \bigcap\limits_{j=1}^{\log n} 
 E_j\right) = \pr \left(E_0 \right) \prod\limits_{j=1}^{\log n} \pr\left(E_j~\vert~\bigcap\limits_{j'=1}^{j-1} E_{j'} \right)=\prod\limits_{j=1}^{\log n} \pr\left(E_j~\vert~E_{j-1}\right).
\end{equation}
In the above equation, we are using $\pr(E_0)=1$. By the definition of $E_0$, $\pr\left(E_0\right)=\pr \left(k_0=I(0,\ell)\right)$.  Note that our algorithms sets $k_0=1$ deterministically. On the other hand, $I(0,\ell)=1$ as (by Definition~\ref{defi:hset}) $[n]$ is the first and only one hierarchical subset of $[n]$ having label $0$. So, $\pr\left(E_0\right)=1$.

By Equation~\ref{eqn:prob-cond}, we can approximate $\pr(k_{\log n}=\ell)$ by approximating $\pr(E_j~\vert ~E_{j-1})=\pr(k_j=I(j,\ell)~\vert ~k_{j-1}=I(j-1,\ell))$ for each $j\in [\log n]$. For that purpose consider the following observation.
 
\begin{obs}\label{obs:iter-j}
Let $j \in [\log n]$ and $\randsamp(i,\alpha,\delta)$ is executing the $j$-th iteration. Also let $k_{j-1}=k^*$. Then for $k^{\#} \in \{2k^*-1,2k^*\}$, 
$$ (1-4\alpha')
\frac{\ham\left(\mat{A}(i,*)\vert_{S_{j}^{k^{\#}}},\mat{B}(i,*)\vert_{S_{j}^{k^{\#}}}\right)}
{\ham\left(\mat{A}(i,*)\vert_{S_{j-1}^{k^{*}}},\mat{B}(i,*)\vert_{S_{j-1}^{k^{*}}}\right)}\leq \pr \left(k_j=k^{\#}\right) \leq (1+4\alpha')
\frac{\ham\left(\mat{A}(i,*)\vert_{S_{j}^{k^{\#}}},\mat{B}(i,*)\vert_{S_{j}^{k^{\#}}}\right)}
{\ham\left(\mat{A}(i,*)\vert_{S_{j-1}^{k^{*}}},\mat{B}(i,*)\vert_{S_{j-1}^{k^{*}}}\right)}.$$
\end{obs}

\begin{proof}
We prove the stated bound for $\pr(k_j=2k^*-1)$ and the proof for $\pr(k_k=2k^*)$ is similar. In the $j$-th iteration $\randsamp(i,\alpha,\delta)$ calls for $\resdistrows \left(S_{j}
^{2k^*-1},i,\alpha',\delta'\right)$ and $\resdistrows \left(S_{j}^{2k^*},i,\alpha',\delta',\right)
$. Let $d_1^j$ and $d_2^j$ be the respective outputs. Then the algorithm sets $k_j=2k^*-1$ with probability $\frac{d_1^j}{d_1^j+d_2^j}$ and $k_j=2k^*$ with the remaining probability. .
 Note that $d_1^j$ and $d_2^j$ are $(1\pm \alpha')$-approximation of $\ham\left(\mat{A}(i,*)\vert_{S_{j}^{2k^{*}-1}},\mat{B}(i,*)\vert_{S_{j}^{2k^{*}-1}}\right)$ and $\ham\left(\mat{A}(i,*)\vert_{S_{j}^{2k^{*}}},\mat{B}(i,*)\vert_{S_{j}^{2k^{*}}}\right)$, respectively. By Observation~\ref{obs:hset} (ii), $S_{j-1}^{k^*}=S_{j}^{2k^*-1} \sqcup S_{j-1}^{2k^*}$. So, 
$$ \ham\left(\mat{A}(i,*)\vert_{S_{j-1}^{k^{*}}},\mat{B}(i,*)\vert_{S_{j-1}^{k^{*}}}\right)=\ham\left(\mat{A}(i,*)\vert_{S_{j}^{2k^{*}-1}},\mat{B}(i,*)\vert_{S_{j}^{2k^{*}-1}}\right)+\ham\left(\mat{A}(i,*)\vert_{S_{j}^{2k^{*}}},\mat{B}(i,*)\vert_{S_{j}^{2k^{*}}}\right).$$
 So, $d_1^j + d_2^j$ is an $(1\pm 2 \alpha')$-approximation to $\ham\left(\mat{A}(i,*)\vert_{S_{j-1}^{k^{*}}},\mat{B}(i,*)\vert_{S_{j-1}^{k^{*}}}\right)$. Hence, $\pr(k_j=2k^*-1)=\frac{d_1^j}{d_1^j+d_2^j}$ can be bounded as
 
\begin{eqnarray*}
\small
&& \left(\frac{1-\alpha'}{1+2\alpha'}\right)\frac{\ham\left(\mat{A}(i,*)\vert_{S_{j}^{k^{\#}}},\mat{B}(i,*)\vert_{S_{j}^{k^{\#}}}\right)}
{\ham\left(\mat{A}(i,*)\vert_{S_{j-1}^{k^{*}}},\mat{B}(i,*)\vert_{S_{j-1}^{k^{*}}}\right)} \leq \pr(k_j=2k^*-1) \leq \left(\frac{1+\alpha'}{1-2\alpha'}\right)\frac{\ham\left(\mat{A}(i,*)\vert_{S_{j}^{k^{\#}}},\mat{B}(i,*)\vert_{S_{j}^{k^{\#}}}\right)}{
\ham\left(\mat{A}(i,*)\vert_{S_{j-1}^{k^{*}}},\mat{B}(i,*)\vert_{S_{j-1}^{k^{*}}}\right)}
\end{eqnarray*}
 Note that we are done with the desired bound for $\pr(k_j=2k^*-1)$.
 %From the description of the algorithm, $\pr(k_j=2k^*-1)\frac{d_1^j}{d_1^j+d_2^j}$. Observe that it lies in the interval as given in the statement because of the approximation guarantee for $d_1^j$ and $d_2^j$ as discussed above. Similarly, one can also argue for  $\pr(k_j=2k^*)$.
\end{proof}

For $\pr(E_j~\vert~E_{j-1})$, take $k^*=I(j-1,\ell)$ and $k^{\#}=I(j,\ell)$ in the above Observation. Then we get 
$$
\pr(E_j~\vert ~E_{j-1}) = \pr\left(k_j=I(j,\ell)~\vert ~ k_{j-1}=I(j-1,\ell)\right) \\
\leq (1+4\alpha')\frac{\ham\left(\mat{A}(i,*)\vert_{S_{j}^{I(j,\ell)}}, \mat{B}(i,*)\vert_{S_{j}^{I(j,\ell)}}\right)}{\ham\left(\mat{A}(i,*)\vert_{S_{j-1}^{I(j-1,\ell)}}, \mat{B}(i,*)\vert_{S_{-1j}^{I(j-1,\ell)}}\right)}.
$$
Putting the above for each $j \in [\log n]$ in Equation~\ref{eqn:prob-cond}, we have 

$$\pr(E_j~\vert ~E_{j-1})= \prod\limits_{j=1}^{\log n}(1+4\alpha')\frac{\ham\left(\mat{A}(i,*)\vert_{S_{j}^{I(j,\ell)}}, \mat{B}(i,*)\vert_{S_{j}^{I(j,\ell)}}\right)}{\ham\left(\mat{A}(i,*)\vert_{S_{j-1}^{I(j-1,\ell)}}, \mat{B}(i,*)\vert_{S_{-1j}^{I(j-1,\ell)}}\right)} \leq (1+4\alpha')^{\log n}\frac{1}{\ham\left(\mat{A}(i,*),\mat{B}(i,*)\right)}.$$

Observe that $\ham\left(\mat{A}(i,*),\mat{B}(i,*)\right)=\size{\mbox{{\sc NEQ}(\mat{A},\mat{B},i)}}$. Also recall that $\alpha'=\frac{\alpha}{50 \log n}$. Hence, we have $\pr(E_j~\vert ~E_{j-1})\leq (1+\alpha)\frac{1}{\size{\mbox{{\sc NEQ}(\mat{A},\mat{B},i)}}}$.

The proof of $\pr(E_j~\vert ~E_{j-1})\geq (1-\alpha)\frac{1}{\size{\mbox{{\sc NEQ}(\mat{A},\mat{B},i)}}}$ is similar.

\end{proof}
%%%%%%%%%%%%%%%%%%%%%End of proof of Lemma 2.8 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> discuss.tex <==

\section{Conclusion}
\label{sec:conclude}
In this paper, we estimated the Hamming distance between two 2-dimensional binary images using projections of a row (or column) of the binary matrix onto a Hamming vector $\{0,1\}^n$ and dimensionality reduction techniques. The next obvious question is to extend this to 3-dimensional binary images. Can random projections of a 2-dimensional image slice onto a Hamming matrix $\{0,1\}^{n \times n}$ and using Johnson Lindenstrauss lemma allow us to estimate the distance between two 3-dimensional binary images? Another important question for imaging tasks is to estimate the distance between two binary images where one image might have undergone a rigid or similarity transform. We also want to study the distance between two 2-dimensional gray-level images.
